Scaling-Up Reasoning and Advanced Analytics on BigData

BigDatalog is an extension of Datalog that achieves performance and scalability on both Apache Spark and multicore systems to the point that its graph analytics outperform those written in GraphX. Looking back, we see how this realizes the ambitious goal pursued by deductive database researchers beginning forty years ago: this is the goal of combining the rigor and power of logic in expressing queries and reasoning with the performance and scalability by which relational databases managed Big Data. This goal led to Datalog which is based on Horn Clauses like Prolog but employs implementation techniques, such as Semi-naive Fixpoint and Magic Sets, that extend the bottom-up computation model of relational systems, and thus obtain the performance and scalability that relational systems had achieved, as far back as the 80s, using data-parallelization on shared-nothing architectures. But this goal proved difficult to achieve because of major issues at (i) the language level and (ii) at the system level. The paper describes how (i) was addressed by simple rules under which the fixpoint semantics extends to programs using count, sum and extrema in recursion, and (ii) was tamed by parallel compilation techniques that achieve scalability on multicore systems and Apache Spark. This paper is under consideration for acceptance in Theory and Practice of Logic Programming (TPLP).

==> analytics.tex <==
\section{Advanced Analytics}\label{sec:analytics}

Beyond the traditional relational and graph applications, our language also enables many advanced analytics applications that seek to extract interesting patterns from data. In the following, we use examples to show how several types of applications can be efficiently expressed, and more examples are available in \cite{yang2017declarative}.

\paragraph{Classification.}
In this type of applications, we seek to extract models from existing data, and use these models to predict class labels for future data. The existing data and future data is often referred to as the training data and testing data, respectively. Assume that the training data is represented as a relation ${\tt train(Id, Col, Val, Cls)}$, where each tuple indicates that the value of the ${\tt Col}$-th feature is ${\tt Val}$ for the tuple with ${\tt Id}$ and class label ${\tt Cls}$. We explain how to build a specific type of classifier called {\em naive Bayes classifier}.

Let $C_1, \cdots, C_m$ be the classes we aim to predict. Let $p(C_i)$ be the {\em prior} probability of class $C_i$, i.e., the probability of having a tuple with class $C_i$ in the training data. For each tuple, let $x_j$ be the value of the $j$-th column, then the {\em likelihood} $p(x_j|C_i)$ is the probability that a tuple with class $C_i$ also having value $x_j$. Given a tuple from the testing data, the classifier predicts a class for the tuple by finding the class $C_i$ that maximizes the {\em posterior}, which is equivalent to maximizing $\log(p(C_i)) + \sum_{j = 1}^k \log(p(x_j|C_i))$. Moreover, assume that we use a multinomial distribution for each likelihood, then $p(x_j|C_i) = {\sf count} \langle {x_j} \rangle / {\sf count} \langle {C_i} \rangle$, where ${\sf count} \langle {x_j} \rangle$ is the number of tuples with the value of the $j$-th column being a specific $x_j$, ${\sf count} \langle {C_i} \rangle$ is the number of tuples with class $C_i$, and both numbers are computed using tuples in the training data. The example below shows how to implement such a classifier in our language.

\begin{example}[A naive Bayes classifier]\label{rule:bayes}
The training data is scanned to count the number of tuples, the prior for each class ${\tt Cls}$, and the number of occurrences for each unique $({\tt Col}, {\tt Val}, {\tt Cls})$ combination. Then the likelihood is computed, and we store the log value in predicate ${\tt likelihood}$.
\begin{displaymath}
\begin{aligned}
& {\tt total(\cntv{Id})} \arrow {\tt train(Id, Col, \_, \_)}, {\tt Col = 1}. \\
& {\tt prior(Cls, \cntv{Id})} \arrow {\tt train(Id, Col, \_, Cls)}, {\tt Col = 1}. \\
& {\tt occur(Col, Val, Cls, \cntv{Id})} \arrow {\tt train(Id, Col, Val, Cls)}. \\
& {\tt likelihood(Col, Val, Cls, P)} \arrow {\tt occur(Col, Val, Cls, C1)}, {\tt prior(Cls, C2)}, \\
& \hspace{14.3em} {\tt P = {\sf log}(C1) - {\sf log}(C2)}.
\end{aligned}
\end{displaymath}
Now assume that ${\tt test(Id, Col, Val)}$ contains the testing data. For each tuple, we compute the posterior for each class, and select the class with higher posterior as the prediction for this tuple.
\begin{displaymath}
\begin{aligned}
& {\tt test\_likelihood(Id, Cls, \sumv{Prob})} \arrow {\tt test(Id, Col, Val)}, \\
& \hspace{18.3em} {\tt likelihood(Col, Val, Cls, Prob)}. \\
& {\tt predict(Id, Cls)} \arrow {\tt test\_likelihood(Id, Cls, Prob)}, {\tt prior(Cls, C)}, {\tt total(CT)}, \\
& \hspace{9.2em} {\tt Prob1 = Prob + {\sf log}(C) - {\sf log}(CT)}, {\tt {\sf is\_max}((Cls), (Prob1))}.
\end{aligned}
\end{displaymath}
\end{example}

\paragraph{Regression Analysis.} Assume that the predicate ${\tt house(Id, Col, Val, Price)}$ stores information about house listings, where each tuple in the relation indicates that the value of the ${\tt Col}$-th feature is ${\tt Val}$ for the house with ${\tt Id}$ and ${\tt Price}$. Moreover, we assume that all these values are numeric. Given a relation like ${\tt house}$, regression analysis can help us learn the relationship between house price and other basic properties, i.e., find a function that takes the values of other basic properties as the input and the output is a predicted house price that is very close to the actual house price provided in the ${\tt house}$ relation.

The example below describes the batch gradient descent algorithm on finding such functions. It performs {\em linear regression}, i.e., the function we want to learn is a linear function that is represented as a $(k + 1)$-dimensional vector, where $k$ is the number of unique values of ${\tt Col}$ in ${\tt house}$. Furthermore, we use a {\em least-squares cost function} to measure how close the predicted house prices are w.r.t. the actual house prices, where the ``closeness'' is defined as the square of the difference between a predicted house price and the actual house price, and the cost function is the average of the ``closeness'' values for all houses in the relation.

\begin{example}[Batch gradient descent]\label{rule:bgd}
We extend the ${\tt house}$ predicate by adding an additional column 0 with a fixed value 1 for every house.
\begin{displaymath}
\begin{aligned}
& {\tt vhouse(Id, Col, Val, Price)} \arrow {\tt house(Id, Col, Val, Price)}. \\
& {\tt vhouse(Id, 0, 1, Price)} \arrow {\tt house(Id, \_, \_, Price)}.
\end{aligned}
\end{displaymath}
We start with an initial model that is a zero vector (or a random vector), and iteratively compute a new model using the model obtained in the previous iteration. For each column ${\tt Col}$, the value of this column in the new model is obtained by adding ${\tt 2.0 / N * LR * G}$ to its current value, where ${\tt N}$ is the total number houses, ${\tt LR}$ is a parameter that represents the learning rate, and ${\tt G}$ is the ${\tt Col}$-th element of the gradient vector.
\begin{displaymath}
\begin{aligned}
& {\tt model(0, Col, 0)} \arrow {\tt vhouse(\_, Col, \_, \_)}. \\
& {\tt model(J1, Col, Val1)} \arrow {\tt model(J, Col, Val)}, {\tt gradient(J, Col, G)}, {\tt parameter(LR)}, \\
& \hspace{10.7em} {\tt housecnt(N)}, {\tt Val1 = Val + 2.0 / N * LR * G}, {\tt J1 = J + 1}. \\
& {\tt gradient(J, Col, \sumv{G})} \arrow {\tt vhouse(Id, Col, Val, Price)}, {\tt cp(J, Id, Predict)}, \\
& \hspace{12.5em} {\tt G = (Price - Predict) * Val}. \\
& {\tt cp(J, Id, \sumv{Prod})} \arrow {\tt vhouse(Id, Col, Val, \_)}, {\tt model(J, Col, Val1)}, \\
& \hspace{10.5em} {\tt Prod = Val * Val1}. \\
& {\tt housecnt(\cntv{Id})} \arrow {\tt vhouse(Id, Col, \_, \_)}, {\tt Col = 0}.
\end{aligned}
\end{displaymath}
\end{example}

\paragraph{Cluster Analysis.}
The goal of cluster analysis is to partition a set of objects into subsets, where each subset is a cluster such that the objects in this cluster are similar to each other while dissimilar to objects in other clusters. We describe an agglomerative hierarchical clustering method that organizes the objects into a hierarchy of clusters by iteratively merging small clusters into a large cluster. We still use the predicate ${\tt house}$ as an example, where each house is now referred to as a point. However, the listing price is no longer a separate column, and is kept in the form of a tuple in ${\tt house(Id, Col, Val)}$.

\begin{example}[AGglomerative NESting (AGNES)]\label{rule:agnes}
Initially, every point is in a cluster of its own, with the point Id as the cluster Id. Then, at each step, we select two clusters ${\tt C1}$ and ${\tt C2}$ such that neither is selected before and the distance between these two clusters (defined in ${\it r9}$) is the smallest. We merge them to create a new cluster ${\tt J + 1}$, where ${\tt J}$ is the current maximal cluster Id. This merge operation is recorded by two tuples ${\tt (J + 1, C1)}$ and ${\tt (J + 1, C2)}$ in ${\tt cluster}$, indicating that cluster ${\tt J + 1}$ is the parent of both cluster ${\tt C1}$ and cluster ${\tt C2}$.
\begin{displaymath}
\begin{aligned}
& {\it r1}.~{\tt cluster(Id, Id)} \arrow {\tt house(Id, Col, Val)}, {\tt Col = 1}. \\
& {\it r2}.~{\tt mc(\fsmaxv{C})} \arrow {\tt cluster(C, \_)}. \\
& {\it r3}.~{\tt merge(J1, C1, C2)} \arrow {\tt mc(J)}, {\tt cluster(C1, \_)}, {\tt cluster(C2, \_)}, {\tt C1 < C2}, \\
& \hspace{10.7em} {\tt {\sf choice}((C1), (J))}, {\tt {\sf choice}((C2), (J))}, {\tt {\sf choice}((J), (C1, C2))}, \\
& \hspace{10.7em} {\tt dc(C1, C2, Dist)}, {\tt {\sf is\_min}((C1, C2), (Dist))},
{\tt J1 = J + 1}. \\
& {\it r4}.~{\tt cluster(J1, C1)} \arrow {\tt merge(J1, C1, \_)}. \\
& {\it r5}.~{\tt cluster(J1, C2)} \arrow {\tt merge(J1, \_, C2)}.
\end{aligned}
\end{displaymath}
These clusters form a hierarchical structure, where the points in a cluster can be found by collecting all the points that belong to its child clusters. Then the distance   ${\tt Dist}$ between two clusters ${\tt C1}$ and ${\tt C2}$ is defined as the minimal Euclidean distance between every pair of points $({\tt Id1}$, ${\tt Id2})$, where ${\tt Id1}$ and ${\tt Id2}$ belong to ${\tt C1}$ and ${\tt C2}$, respectively.
\begin{displaymath}
\begin{aligned}
& {\it r6}.~{\tt cp(Id, Id)} \arrow {\tt cluster(Id, Id)}. \\
& {\it r7}.~{\tt cp(C, Id)} \arrow {\tt cluster(C, C1)}, {\tt cp(C1, Id)}. \\
& {\it r8}.~{\tt dp(Id1, Id2, \sumv{D})} \arrow {\tt house(Id1, Col, V1)}, {\tt house(Id2, Col, V2)}, \\
&\hspace{12em} {\tt D = (V1 - V2) * (V1 - V2)}. \\
& {\it r9}.~{\tt dc(C1, C2, \minv{Dist})} \arrow {\tt cp(C1, Id1)}, {\tt cp(C2, Id2)}, {\tt dp(Id1, Id2, Dist)}.
\end{aligned}
\end{displaymath}
\end{example} 

==> analytics2.tex <==
\section{Advanced Analytics}\label{sec:analytics}

Beyond the traditional relational and graph applications, our language also enables many advanced analytics applications.
Many of these applications can be supported with XY-stratifications \cite{scalingdatalog} or simple aggregates. For example, using simple aggregates we can perform advanced applications like Naive Bayesian classification and with XY stratification we can perform even more complicated tasks like regression and clustering. These examples are discussed later in the Appendix. 

In this section, we focus more on certain advanced data mining applications which can leverage the optimization strategies discussion in Section \ref{sec:extrema}. For this, we introduce the notion of prefix tables and data cubes that play a central role in many data mining applications like frequent itemset mining or iceberg query execution. 


\subsection{Prefix Table}\label{sec:prefixtable}

Consider the well-known {\em PlayTennis} example from \cite{mitchell1997machine} \ctab\ref{tab:train}. 
Analytic tasks written with this table in mind cannot be easily applied on other tables which has different number of columns and data types. Therefore, in order to ensure genericity, we consider the equivalent vertical representation of the table which has a column indicating the column number from the original table and another column to capture the values for the tuples.  
For example, \ctab\ref{tab:vtrain} presents the verticalized view of the {\em PlayTennis} example.

\begin{table*}[h]
\begin{minipage}[t]{0.65\linewidth}
\centering
\caption{Training examples for\\ the PlayTennis table.}\label{tab:train}
%\vspace{-1em}
{\small
 \begin{tabular}{|@{\hspace{0.1em}}c@{\hspace{0.1em}}|c|@{\hspace{0.1em}}c@{\hspace{0.1em}}|@{\hspace{0.1em}}c@{\hspace{0.1em}}|c|@{\hspace{0.1em}}c@{\hspace{0.1em}}|}
 \hline
 \multirow{2}{*}{\bf ID} & \multirow{2}{*}{\bf Outlook} & {\bf Tempe} & \multirow{2}{*}{\bf Humidity} & \multirow{2}{*}{\bf Wind} & {\bf Play} \\
 & & {\bf rature} & & & {\bf Tennis} \\
 & (1) & (2) & (3) & (4) & (5) \\
 \hline
 \hline
 1	 & sunny     & hot		 & high      & weak      & no \\
 2	 & sunny     & hot		 & high		 & strong    & no \\
 3	 & overcast	 & hot		 & high		 & weak	     & yes \\
 4	 & rain		 & mild		 & high		 & weak	     & yes \\
 5	 & rain		 & cool		 & normal	 & weak      & yes \\
 6	 & rain		 & cool		 & normal	 & strong    & no \\	
 7	 & overcast	 & cool		 & normal	 & strong    & yes \\	
 8	 & sunny	 & mild		 & high		 & weak      & no \\	
 9	 & sunny     & cool		 & normal	 & weak      & yes \\
 10	 & rain		 & mild		 & normal	 & weak      & yes \\	
 11	 & sunny     & mild      & normal	 & strong    & yes \\	
 12	 & overcast	 & mild		 & high		 & strong    & yes \\	
 13	 & overcast	 & hot		 & normal	 & weak      & yes \\	
 14	 & rain		 & mild		 & high		 & strong    & no \\
 \hline
\end{tabular}
}
\end{minipage}
\end{table*}

%\hfill
\begin{table*}[h]
\begin{minipage}[t]{0.5\linewidth}
\centering
\captionsetup{justification=centering}
\caption{Vertical view of the tuples in \ctab\ref{tab:train}.}\label{tab:vtrain}
%\vspace{-1em}
{\small
 \begin{tabular}{|@{\hspace{0.1em}}c@{\hspace{0.1em}}|@{\hspace{0.1em}}c@{\hspace{0.1em}}|c|}
 \hline
 {\bf ID} & {\bf Col} & {\bf Val} \\
 \hline \hline
 1	 & 1     & sunny \\	
 1	 & 2  	 & hot \\	
 1	 & 3     & high	\\	
 1	 & 4     & weak \\
 1   & 5     & no \\
 2	 & 1     & sunny \\
 2	 & 2     & hot \\	
 2	 & 3     & high \\	
 2	 & 4     & strong \\
 2	 & 5     & no \\		
 3	 & 1     & overcast \\	
 3   & 2     & hot \\	
 3   & 3     & high \\
 3   & 4     & weak \\
 3   & 5     & yes \\
 $\ldots$ & $\ldots$ & $\ldots$ \\
% 4 &5 &Rain \\	
% 4 & 2  &Mild& 1\\	
% 4 &3  & High	& 1\\
% 4 & 4  & Weak	& 1\\
% 5 &1 &Rain &1\\	
% 5 & 2  &Cool& 1\\	
% 5 &3  & Normal & 1\\
% 5 & 4  & Weak	& 1\\
% 6 &1 &Rain &0\\	
% 6 & 2  &Cool&  0\\	
% 6 &3 & Normal & 0\\
% 6  & 4  &  Strong	& 0\\
% 7 & etc. & etc. & etc.
 \end{tabular}
}
\end{minipage}
%\hfill
%\vspace{-1em}
\end{table*}

Additionally, sometimes many applications like supervised classification have labelled tuples. For such labelled datasets, an alternative vertical representation is shown in \ctab\ref{tab:vtrain2} where the class label is not verticalized as other attribute columns. 

\begin{table*}[h]
\begin{minipage}[t]{0.75\linewidth}
\centering
\captionsetup{justification=centering}
\caption{An alternative vertical representation treating class label and attribute columns separately.}\label{tab:vtrain2}
%\vspace{-1em}
{\small
 \begin{tabular}{|@{\hspace{0.1em}}c@{\hspace{0.1em}}|@{\hspace{0.1em}}c@{\hspace{0.1em}}|c|@{\hspace{0.1em}}c@{\hspace{0.1em}}|}
 \hline
 \multirow{2}{*}{\bf ID} & \multirow{2}{*}{\bf Col} & \multirow{2}{*}{\bf Val} & {\bf Play} \\
 & & & {\bf Tennis} \\
 \hline \hline
 1	 & 1     & sunny & no \\	
 1	 & 2  	 & hot & no \\	
 1	 & 3     & high	& no \\	
 1	 & 4     & weak & no \\
 2	 & 1     & sunny & no \\
 2	 & 2     & hot & no \\	
 2	 & 3     & high & no \\	
 2	 & 4     & strong & no \\
 3	 & 1     & overcast & yes \\	
 3   & 2     & hot & yes \\	
 3   & 3     & high & yes \\
 3   & 4     & weak & yes \\
 $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
 \end{tabular}
}
\end{minipage}
%\hfill
%\vspace{-1em}
\end{table*}


Although vertical representation allows tremendous genericity, it still requires a lot of storage overhead. 
Therefore, we discuss next a more compact representation, following the ideas of basic \texttt{SQL-2003 rollup} that incurs a low storage overhead and provides a reduced computational time. 

The \texttt{SQL-2003 count rollup} aggregate on the previous example in \ctab\ref{tab:train} yields the output in \ctab\ref{tab:table3}.
We limit the output to first 14 lines only.
% once the result is displayed using  {\sc row\_number}, {\sc asc}, {\sc nulls first} (to save space we only show the first 14 lines among the 51 lines in total).

\begin{table*}[t]
\centering
\caption{The count rollup for the example in \ctab\ref{tab:train}.}\label{tab:table3}
%\vspace{-1em}
{\small
 \begin{tabular}{|c|c|c|c|c|c|c|}
 \hline
 {\bf ID} & {\bf Outlook} & {\bf Temperature} & {\bf Humidity} & {\bf Wind} & {\bf PlayTennis} & {\bf count} \\
 & (1) & (2) & (3) & (4) & (5) & \\
 \hline \hline
 1	 & \textcolor{red}{null}		 & null		 & null	 & null	 & null & 14 \\
 2	 & \textcolor{red}{overcast}	 & null		 & null	 & null	 & null & 4 \\
 3	 & overcast	 & \textcolor{red}{cool}		 & null	 & null	 & null & 1 \\
 4	 & overcast	 & cool		 & \textcolor{red}{normal}	 & null	 & null & 1 \\
 5	 & overcast	 & cool		 & normal	 &  \textcolor{red}{strong}	& null & 1 \\
 6	 & overcast	 & cool		 & normal	 &  strong	& \textcolor{red}{yes} & 1 \\
 7	 & overcast	 & \textcolor{red}{hot}		 & null	 & null	 & null & 2 \\
 8	 & overcast	 & hot		 & \textcolor{red}{high}       &null & null & 1 \\
 9	 & overcast	 & hot		 & high       & \textcolor{red}{weak} & null& 1 \\
 10	 & overcast	 & hot		 & high       &weak & \textcolor{red}{yes} & 1 \\
 11	 & overcast	 & \textcolor{red}{mild}		 &null       &null  & null & 1 \\
 12	 & overcast	 & mild 		 & \textcolor{red}{high}       &null  & null & 1 \\
 13	 & overcast	 & mild 		 & high       & \textcolor{red}{strong}  & null & 1 \\
 14	 & overcast	 & mild 		 & high       &strong  & \textcolor{red}{yes} & 1 \\
 $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$
\end{tabular}
}
\end{table*}

However notice that the output of \texttt{rollup} contains many redundant \texttt{null} values and that 
only the items in the main diagonal hold new information  (highlighted in red). 
In fact, the items to left of the diagonal are repeating the previous values (i.e. sharing the prefix), whereas those to right are \texttt{nulls}. 
With this observation, we can compact the \ctab\ref{tab:table3} to a more logically concise representation shown in \ctab\ref{tab:table4}, where the first four columns contain the same information as an item in the main diagonal does, %the ID of the tuple has been placed in the fourth column,
whereas the last column (PID) specifies the ID of the parent tuple from where we can find the value of the previous column. We refer to this condensed representation as a {\em prefix table}. In this particular case it is a {\em rollup prefix table} for count, and similar representations can be used for other aggregates.


\begin{table*}[t]
\begin{minipage}[t]{0.5\linewidth}
\centering
\caption{A rollup prefix table for the tuples in \ctab\ref{tab:table3}.}\label{tab:table4}
%\vspace{-1em}
{\small
 \begin{tabular}{|c|c|c|c|c|}
 \hline
 {\bf ID} & {\bf Col} & {\bf Val} & {\bf count} & {\bf PID}\\
 \hline\hline
 1  & 1 & null      & 14 & 1\\
 2  & 1 & overcast  & 4 & 1\\
 3  & 2 & cool      & 1 & 2\\
 4  & 3 & normal	& 1 & 3\\
 5  & 4 & strong	& 1 & 4\\
 6  & 5 & yes       & 1 & 5\\
 7  & 2 & hot       & 2 & 2\\
 8  & 3 & high      & 1 & 7\\
 9  & 4 & weak      & 1 & 8\\
 10  & 5 & yes      & 1 & 9\\
 11  & 2 & mild     & 1 & 2\\
 12 & 3 & high      & 1 & 11\\
 13 & 4 & strong    & 1 & 12\\
 14 & 5 & yes       & 1 & 13\\
 $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$
\end{tabular}
}
\end{minipage}
\end{table*}

A easier way to understand and visualize \ctab\ref{tab:table4} is through the logically equivalent and more user intuitive 
representation shown in \ctab\ref{tab:table4a}.

\begin{table*}
\begin{minipage}[t]{0.5\linewidth}
\centering
\caption{A logically equivalent and more intuitive rollup prefix table of \ctab\ref{tab:table4}.}\label{tab:table4a}
%\vspace{-1em}
{\small
 \begin{tabular}{|c|c|c|c|c|}
 \hline
 {\bf ID} & {\bf Col} & {\bf Val} & {\bf count} & {\bf PID}\\
 \hline\hline
 1  & 1 & null      & 14 & 1\\
 3  & 1 & overcast  & 4 & 1\\
 7  & 2 & cool      & 1 & 3\\
 7  & 3 & normal	& 1 & 7\\
 7  & 4 & strong	& 1 & 7\\
 7  & 5 & yes       & 1 & 7\\
 3  & 2 & hot       & 2 & 3\\
 3  & 3 & high      & 1 & 3\\
 3  & 4 & weak      & 1 & 3\\
 3  & 5 & yes      & 1 & 3\\
 12 & 2 & mild     & 1 & 3\\
 12 & 3 & high      & 1 & 12\\
 12 & 4 & strong    & 1 & 12\\
 12 & 5 & yes       & 1 & 12\\
 $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$
\end{tabular}
}
\end{minipage}
\end{table*}

The rollup prefix tables for count are just relational representations for prefix trees, which
proved very valuable in data mining algorithms, such as the famous FP-growth algorithm~\cite{han2000mining}. The nodes of rollup prefix tables are identified by integers. 

%In \ctab\ref{tab:table4} the integers form a sequence of consecutive integers. %that corresponds to the preorder traversal of the tree.
%However in general, no logical significance needs to be associated to those numbers: the only requirement is that no two nodes are assigned the same identifier, i.e., the combination of (ID, Col, Val, PID) must be unique. In fact, we can reuse the IDs of the original tuples in \ctab\ref{tab:train}, and one such example is shown in \ctab\ref{tab:table4_1}.
%The corresponding rollup prefix table representation of \ctab\ref{tab:table5} can be obtained from the verticalized representation ${\tt vtrain(T, C, V)}$ using the following rules.
%The example below shows how to construct the corresponding

The rollup prefix table can be constructed from a verticalized representation (say \texttt{vtrain}) using monotonic aggregates as shown below, using the following rules \cite{yang2017declarative}:

\begin{displaymath}
\begin{aligned}
& r1: {\tt repr(T1, C, V, T)} \arrow {\tt vtrain(T, C, V)}, {\tt C = 1}, {\tt T1 = 1}. \\
& r2: {\tt repr(T1, C, V, T)} \arrow {\tt vtrain(T, C, V)}, {\tt C1 = C - 1}, {\tt repr(Ta, C1, V1, T)}, {\tt rupt(T1, C1, V1, \_, Ta)}. \\
& r3: {\tt rupt(\fsminv{T}, C, V, \fscntv{T}, Ta)} \arrow {\tt repr(Ta, C, V, T)}. \\
\end{aligned}
\end{displaymath}
%The rule below is the extraction rule that gets the final values of the monotonic aggregates for each unique combination of ${\tt (Ta, C, V)}$.
%\inv
\begin{displaymath}
r4: {\tt rupt2(\minv{T}, C, V, \maxv{CT}, Ta)} \arrow {\tt rupt(T, C, V, CT, Ta)}. \\
\end{displaymath}
%Note that ${\tt rupt2}$ might contain more tuples than the final rollup prefix table since (i) the continuous monotonic aggregates might produce multiple tuples of the form $(\tt T, C, V, CT, Ta)$ for each unique combination of ${\tt (Ta, C, V)}$, and (ii) these ${\tt T}$ values then become the parent IDs of some tuples in ${\tt repr}$, ${\tt rupt}$, and ${\tt rupt2}$. However, it is easy to see that these parent IDs share the same ${\tt T}$ value in ${\tt rupt2}$. Thus, $r\ref{rule:pt1}.5$ is added to keep the minimal parent ID ${\tt Ta}$, i.e., to keep a unique parent for every node. This rule is not necessary if the tuples in ${\tt vtrain}$ are accessed in increasing order of IDs. This condition is guaranteed since ${\tt vtrain}$ is produced by our built-in verticalization function.
%\inv
\begin{displaymath}
r5: {\tt rupt3(T, C, V, CT, Ta)} \arrow {\tt rupt2(T, C, V, CT, Ta)}, {\tt {\sf is\_min}((T, C, V), (Ta))}.
\end{displaymath}

The operational details of the above program is explained in \cite{yang2017declarative}. 
The rollup prefix tree computed following the semi-naive evaluation and repeated lookups require multiple scans of the tuples and is hence computationally inefficient. However, a a further optimized version with \texttt{if-else} constructs can build the same prefix tree in a single scan. To conceal the complexities, we introduce a built-in aggregate \texttt{rollup} that computes the rollup prefix tree in same time and space complexity as a procedural program from a verticalized representation. An example is shown below:


\begin{displaymath}
{\tt myrupt({\sf rollup} \langle ID \rangle, Col, Val, \cntv{ID}, {\sf prev} \langle ID \rangle)} \arrow {\tt vtrain(ID, Col, Val)}.
\end{displaymath}

In this built-in construct, the keyword ${\sf rollup}$ indicates that we are computing a rollup prefix table, ${\sf rollup} \langle {\tt ID} \rangle$ denotes the operation that selects a representative among all the tuples with the same combination of (PID, Col, Val), and ${\sf prev} \langle {\tt ID} \rangle$ denotes the corresponding operation that decides the PID of a tuple based on the actual implementation of ${\sf rollup} \langle {\tt ID} \rangle$. We have used the $\fsmin$/${\sf min}$ aggregates to implement ${\sf rollup} \langle {\tt ID} \rangle$ in \cexp\ref{rule:pt1}. Other constructs, such as $\fsmax$/${\sf max}$ and ${\sf choice}$, could also be used to deliver logically equivalent rollup prefix tables.

%An algorithm to construct a rollup prefix table from a verticalized representation ${\tt vtrain(T, C, V)}$ (${\tt T}$, ${\tt C}$, and ${\tt V}$ stand for the ID column, Col column, and Val column, respectively) is presented in the example below.\footnote{Hereafter, a rollup prefix table does not contain the tuple that represents the total number of tuples, i.e., the tuple (1, 1, null, 14, 1) in \ctab\ref{tab:table4} and \ctab\ref{tab:table4_1}.}
%which uses a self-explanatory horizontal representation. In this representation, each item $e$ that is not under the ID column and is not empty represents a tuple in the rollup prefix table, where the values for ID, Col, Val, count columns are the tuple ID of $e$, $e$'s column number, $e$'s value, and the number associated with $e$'s value, respectively, and the value of the PID column is determined as follows: if the column number of $e$ equals 1, then PID equals 1; if the item before $e$ is not empty, then PID equals ID; otherwise PID equals the tuple ID of the first non-empty item above $e$. We refer to this representation as a {\em compact rollup} (for count in our example). The compact rollup in \ctab\ref{tab:table5} represents the 51 tuples in \ctab\ref{tab:table3} (excluding the first tuple that shows the total number of tuples) by only 14 tuples. It is easy to see that this representation displays the same information in a more concise and appealing way to end-users w.r.t. the typical rollup output format displayed in \ctab\ref{tab:table3}.

%where each row corresponds to the tuple with the same ID in \ctab\ref{tab:train}. We say that a cell $\mathit{OC}$ can be represented by another cell $\mathit{UC}$ of the same column $\mathit{Col}$ if the corresponding tuples for $\mathit{OC}$ and $\mathit{UC}$ in \ctab\ref{tab:train} are identical in the first $\mathit{Col}$ columns. It is easy to see that this defines an equivalence relation. For each equivalence class, the cell with the smallest tuple ID is selected as an representative to represent the remaining cells, and the remaining cells that do not hold new information are omitted by showing an empty cell in \ctab\ref{tab:table5}. For each omitted cell $\mathit{OC}$, its original value can be recovered as follows: find the closest non-omitted cell $\mathit{UC}$ that is in the same column as $\mathit{OC}$, and above the row of $\mathit{OC}$, then the original value of $\mathit{OC}$ equals the value of $\mathit{UC}$, and the count value in $\mathit{UC}$ indicates the number of cells represented by $\mathit{UC}$ (including itself). In \ctab\ref{tab:table5}, each non-omitted cell $\mathit{UC}$ not in the ID column represents a tuple in the rollup PT, whose ID is the same as the tuple ID of $\mathit{UC}$, and PID is determined as follows: let $\mathit{Col}$ be the column of $\mathit{UC}$, if $\mathit{Col}$ is 1, then PID equals ID, otherwise PID equals the ID of the closet non-omitted cell that is in column $\mathit{Col} - 1$, and in the same row or above the row of $\mathit{UC}$. We refer to this representation as {\em Compact Rollup} (for count in our example). The compact rollup in \ctab\ref{tab:table5} represents the 51 tuples in \ctab\ref{tab:table3} (excluding the first tuple) by only 14 tuples. Our past experience of browsing through pages and pages of output returned by rollups and data cube queries suggests that these compact rollups will be very attractive to end-users. Therefore, we will support this improved representations for descriptive OLAPs and we will also provide constructs to map between various representations, and in particular to and from PT representations such as that in \ctab\ref{tab:table4}. PT representations are in fact generic and provide a natural link between description analytics to discovery analytics. As such, they represent a key feature of our Datalog extension that we will name {\em 3DLog}, for Description \& Discovery DataLog. Some important features of {\em 3DLog} are discussed next.

Similar to the rollup, the \texttt{SQL-2003 count cube} aggregate can also be computed efficiently from the rollup prefix table \cite{yang2017declarative}. 
A cube (from hereon, referred as a cube prefix table) is essentially a prefix tree, with all permutations of attributes. 
A limited example of the cube is shown in \ctab\ref{tab:tablecube}.
We conceal the complexity of cube prefix tree computation from rollup prefix tree with  the following construct that indicates the computation of a data cube directly from ${\tt vtrain}$, where ${\sf cube} \langle {\tt ID} \rangle$ tells the compiler that we are dealing with a data cube.

\begin{displaymath}
{\tt mycpt({\sf cube} \langle ID \rangle, Col, Val, \cntv{ID}, {\sf prev} \langle ID \rangle)} \arrow {\tt vtrain(ID, Col, Val)}.
\end{displaymath}


\begin{table}[htbp]
\centering
\caption{A compact data cube}
\label{tab:tablecube}
%\vspace{-1em}
{\small
 \begin{tabular}{|r|cc|cc|cc|cc|cc|}
 \hline
 %\multirow{2}{*}{\bf ID} & \multirow{2}{*}{\bf Outlook} & \multirow{2}{*}{C1} & {\bf Tempe} & \multirow{2}{*}{C2} & \multirow{2}{*}{\bf Humidity} & \multirow{2}{*}{C3} & \multirow{2}{*}{\bf Wind} & \multirow{2}{*}{C4} & {\bf Play} & \multirow{2}{*}{C5} \\
 %& & & {\bf rature} & & & & & & {\bf Tennis} & \\
 {\bf ID} & {\bf Outlook} & {C1} & {\bf Temperature} & {C2} & {\bf Humidity} & {C3} & {\bf Wind} & {C4} & {\bf PlayTennis} & {C5} \\
 \hline \hline
 1 & sunny & 5 & hot & 2 & high & 2 & weak & 1 & no & 1\\
 2 &   &   &   &   &   &   & strong & 1 & no & 1\\
 8 &   &   & mild & 2 & high & 1 & weak & 1 & no & 1\\
 11 &   &   &   &   & normal & 1 & strong & 1 & yes & 1\\
 9 &   &   & cool & 1 & normal & 1 & weak & 1 & yes & 1\\
 3 & overcast & 4 & hot & 2 & high & 1 & weak & 1 & yes & 1\\
 13 &   &   &   &   & normal & 1 & weak & 1 & yes & 1\\
 7 &   &   & cool & 1 & normal & 1 & strong & 1 & yes & 1\\
 12 &   &   & mild & 1 & high & 1 & strong & 1 & yes & 1\\		
 4 & rain & 5 & mild & 3 & high & 2 & weak & 1 & yes & 1\\
 14 &   &   &   &   &   &   & strong & 1 & no & 1\\
 10 &   &   &   &   & normal & 1 & weak & 1 & yes & 1\\
 5 &   &   & cool & 2 & normal & 2 & weak & 1 & yes & 1\\
 6 &   &   &   &   &   &   & strong & 1 & no & 1\\
 %\cdashline{2-11}
 1(+14) &  null &  14 &  hot &  4 &  high &  3 &  weak &  2 &  no &  1\\
 3(+14) &   &   &   &   &   &   &   &   &  yes &  1\\
 2(+14) &   &   &   &   &   &   &  strong &  1 &  no &  1\\
 13(+14) &   &   &   &   &  normal &  1 &  weak &  1 &  yes &  1\\
 4(+14) &   &   &  mild &  6 &  high &  4 &  weak &  2 &  yes &  1\\
 8(+14) &   &   &   &   &   &   &   &   &  no &  1\\
 12(+14) &   &   &   &   &   &   &  strong &  2 &  yes &  1\\
 14(+14) &   &   &   &   &   &   &   &   &  no &  1\\
 10(+14) &   &   &   &   &  normal &  2 &  weak &  1 &  yes &  1\\
 11(+14) &   &   &   &   &   &   &  strong &  1 &  yes &  1\\
 5(+14) &   &   &  cool &  4 &  normal &  4 &  weak &  2 &  yes &  2\\
 6(+14) &   &   &   &   &   &   & strong &  2 &  no &  1\\
 7(+14) &   &   &   &   &   &   &   &   &  yes &  1\\
 \hline
\end{tabular}
}
\end{table}




\paragraph{Iceberg Queries.}
%We have presented several optimizations for finding frequent item sets with a variable-length representation of paths, such as pruning the computation of nodes that do not carry new information, re-ordering of columns, and controlling the tuple derivation order. These optimizations can also be applied to many other tasks that perform the cube computation using a fixed-length representation of paths. In particular, they can be applied to the computation of
{\em iceberg cubes}~\cite{Fang98computingiceberg}, compute aggregate functions over different set of attributes to find aggregate values above pre-defined thresholds. For example, an iceberg cube that finds all the nodes with count values no less than a predefined threshold can be be computed from the cube prefix tree as below:

\begin{displaymath}
{\tt icebergcpt(ID, Col, Val, Cnt, PID)} \arrow {\tt mycpt(ID, Col, Val, Cnt, PID)}, {\tt threshold(T)}, {\tt Cnt \geq T}.
\end{displaymath}

Our algorithm computes the iceberg cube by constructing a cube prefix table from the rollup prefix table representation of the data set, and checking if the minimal support constraint is satisfied for each node in the cube immediately after the corresponding tuple is derived.

%\paragraph{Frequent Itemset Mining.}


\paragraph{Classification.}
In this type of applications, we seek to extract models from existing data, and use these models to predict class labels for future data. The existing data and future data is often referred to as the training data and testing data, respectively. Assume that the training data is represented as a relation ${\tt train(Id, Col, Val, Cls)}$, where each tuple indicates that the value of the ${\tt Col}$-th feature is ${\tt Val}$ for the tuple with ${\tt Id}$ and class label ${\tt Cls}$. We explain how to build a specific type of classifier called {\em naive Bayes classifier}.

Let $C_1, \cdots, C_m$ be the classes we aim to predict. Let $p(C_i)$ be the {\em prior} probability of class $C_i$, i.e., the probability of having a tuple with class $C_i$ in the training data. For each tuple, let $x_j$ be the value of the $j$-th column, then the {\em likelihood} $p(x_j|C_i)$ is the probability that a tuple with class $C_i$ also having value $x_j$. Given a tuple from the testing data, the classifier predicts a class for the tuple by finding the class $C_i$ that maximizes the {\em posterior}, which is equivalent to maximizing $\log(p(C_i)) + \sum_{j = 1}^k \log(p(x_j|C_i))$. Moreover, assume that we use a multinomial distribution for each likelihood, then $p(x_j|C_i) = {\sf count} \langle {x_j} \rangle / {\sf count} \langle {C_i} \rangle$, where ${\sf count} \langle {x_j} \rangle$ is the number of tuples with the value of the $j$-th column being a specific $x_j$, ${\sf count} \langle {C_i} \rangle$ is the number of tuples with class $C_i$, and both numbers are computed using tuples in the training data. The example below shows how to implement such a classifier in our language.

\begin{example}[A naive Bayes classifier]\label{rule:bayes}
The training data is scanned to count the number of tuples, the prior for each class ${\tt Cls}$, and the number of occurrences for each unique $({\tt Col}, {\tt Val}, {\tt Cls})$ combination. Then the likelihood is computed, and we store the log value in predicate ${\tt likelihood}$.
\begin{displaymath}
\begin{aligned}
& {\tt total(\cntv{Id})} \arrow {\tt train(Id, Col, \_, \_)}, {\tt Col = 1}. \\
& {\tt prior(Cls, \cntv{Id})} \arrow {\tt train(Id, Col, \_, Cls)}, {\tt Col = 1}. \\
& {\tt occur(Col, Val, Cls, \cntv{Id})} \arrow {\tt train(Id, Col, Val, Cls)}. \\
& {\tt likelihood(Col, Val, Cls, P)} \arrow {\tt occur(Col, Val, Cls, C1)}, {\tt prior(Cls, C2)}, \\
& \hspace{14.3em} {\tt P = {\sf log}(C1) - {\sf log}(C2)}.
\end{aligned}
\end{displaymath}
Now assume that ${\tt test(Id, Col, Val)}$ contains the testing data. For each tuple, we compute the posterior for each class, and select the class with higher posterior as the prediction for this tuple.
\begin{displaymath}
\begin{aligned}
& {\tt test\_likelihood(Id, Cls, \sumv{Prob})} \arrow {\tt test(Id, Col, Val)}, \\
& \hspace{18.3em} {\tt likelihood(Col, Val, Cls, Prob)}. \\
& {\tt predict(Id, Cls)} \arrow {\tt test\_likelihood(Id, Cls, Prob)}, {\tt prior(Cls, C)}, {\tt total(CT)}, \\
& \hspace{9.2em} {\tt Prob1 = Prob + {\sf log}(C) - {\sf log}(CT)}, {\tt {\sf is\_max}((Cls), (Prob1))}.
\end{aligned}
\end{displaymath}
\end{example}

%   \subsection{XY Stratification based analytics}
% % \paragraph{Regression Analysis.} Assume that the predicate ${\tt house(Id, Col, Val, Price)}$ stores information about house listings, where each tuple in the relation indicates that the value of the ${\tt Col}$-th feature is ${\tt Val}$ for the house with ${\tt Id}$ and ${\tt Price}$. Moreover, we assume that all these values are numeric. Given a relation like ${\tt house}$, regression analysis can help us learn the relationship between house price and other basic properties, i.e., find a function that takes the values of other basic properties as the input and the output is a predicted house price that is very close to the actual house price provided in the ${\tt house}$ relation.

% The example below describes the batch gradient descent algorithm on finding such functions. It performs {\em linear regression}, i.e., the function we want to learn is a linear function that is represented as a $(k + 1)$-dimensional vector, where $k$ is the number of unique values of ${\tt Col}$ in ${\tt house}$. Furthermore, we use a {\em least-squares cost function} to measure how close the predicted house prices are w.r.t. the actual house prices, where the ``closeness'' is defined as the square of the difference between a predicted house price and the actual house price, and the cost function is the average of the ``closeness'' values for all houses in the relation.

% \begin{example}[Batch gradient descent]\label{rule:bgd}
% We extend the ${\tt house}$ predicate by adding an additional column 0 with a fixed value 1 for every house.
% \begin{displaymath}
% \begin{aligned}
% & {\tt vhouse(Id, Col, Val, Price)} \arrow {\tt house(Id, Col, Val, Price)}. \\
% & {\tt vhouse(Id, 0, 1, Price)} \arrow {\tt house(Id, \_, \_, Price)}.
% \end{aligned}
% \end{displaymath}
% We start with an initial model that is a zero vector (or a random vector), and iteratively compute a new model using the model obtained in the previous iteration. For each column ${\tt Col}$, the value of this column in the new model is obtained by adding ${\tt 2.0 / N * LR * G}$ to its current value, where ${\tt N}$ is the total number houses, ${\tt LR}$ is a parameter that represents the learning rate, and ${\tt G}$ is the ${\tt Col}$-th element of the gradient vector.
% \begin{displaymath}
% \begin{aligned}
% & {\tt model(0, Col, 0)} \arrow {\tt vhouse(\_, Col, \_, \_)}. \\
% & {\tt model(J1, Col, Val1)} \arrow {\tt model(J, Col, Val)}, {\tt gradient(J, Col, G)}, {\tt parameter(LR)}, \\
% & \hspace{10.7em} {\tt housecnt(N)}, {\tt Val1 = Val + 2.0 / N * LR * G}, {\tt J1 = J + 1}. \\
% & {\tt gradient(J, Col, \sumv{G})} \arrow {\tt vhouse(Id, Col, Val, Price)}, {\tt cp(J, Id, Predict)}, \\
% & \hspace{12.5em} {\tt G = (Price - Predict) * Val}. \\
% & {\tt cp(J, Id, \sumv{Prod})} \arrow {\tt vhouse(Id, Col, Val, \_)}, {\tt model(J, Col, Val1)}, \\
% & \hspace{10.5em} {\tt Prod = Val * Val1}. \\
% & {\tt housecnt(\cntv{Id})} \arrow {\tt vhouse(Id, Col, \_, \_)}, {\tt Col = 0}.
% \end{aligned}
% \end{displaymath}
%\end{example}

% \paragraph{Cluster Analysis.}
% The goal of cluster analysis is to partition a set of objects into subsets, where each subset is a cluster such that the objects in this cluster are similar to each other while dissimilar to objects in other clusters. We describe an agglomerative hierarchical clustering method that organizes the objects into a hierarchy of clusters by iteratively merging small clusters into a large cluster. We still use the predicate ${\tt house}$ as an example, where each house is now referred to as a point. However, the listing price is no longer a separate column, and is kept in the form of a tuple in ${\tt house(Id, Col, Val)}$.

% \begin{example}[AGglomerative NESting (AGNES)]\label{rule:agnes}
% Initially, every point is in a cluster of its own, with the point Id as the cluster Id. Then, at each step, we select two clusters ${\tt C1}$ and ${\tt C2}$ such that neither is selected before and the distance between these two clusters (defined in ${\it r9}$) is the smallest. We merge them to create a new cluster ${\tt J + 1}$, where ${\tt J}$ is the current maximal cluster Id. This merge operation is recorded by two tuples ${\tt (J + 1, C1)}$ and ${\tt (J + 1, C2)}$ in ${\tt cluster}$, indicating that cluster ${\tt J + 1}$ is the parent of both cluster ${\tt C1}$ and cluster ${\tt C2}$.
% \begin{displaymath}
% \begin{aligned}
% & {\it r1}.~{\tt cluster(Id, Id)} \arrow {\tt house(Id, Col, Val)}, {\tt Col = 1}. \\
% & {\it r2}.~{\tt mc(\fsmaxv{C})} \arrow {\tt cluster(C, \_)}. \\
% & {\it r3}.~{\tt merge(J1, C1, C2)} \arrow {\tt mc(J)}, {\tt cluster(C1, \_)}, {\tt cluster(C2, \_)}, {\tt C1 < C2}, \\
% & \hspace{10.7em} {\tt {\sf choice}((C1), (J))}, {\tt {\sf choice}((C2), (J))}, {\tt {\sf choice}((J), (C1, C2))}, \\
% & \hspace{10.7em} {\tt dc(C1, C2, Dist)}, {\tt {\sf is\_min}((C1, C2), (Dist))},
% {\tt J1 = J + 1}. \\
% & {\it r4}.~{\tt cluster(J1, C1)} \arrow {\tt merge(J1, C1, \_)}. \\
% & {\it r5}.~{\tt cluster(J1, C2)} \arrow {\tt merge(J1, \_, C2)}.
% \end{aligned}
% \end{displaymath}
% These clusters form a hierarchical structure, where the points in a cluster can be found by collecting all the points that belong to its child clusters. Then the distance ${\tt Dist}$ between two clusters ${\tt C1}$ and ${\tt C2}$ is defined as the minimal Euclidean distance between every pair of points $({\tt Id1}$, ${\tt Id2})$, where ${\tt Id1}$ and ${\tt Id2}$ belong to ${\tt C1}$ and ${\tt C2}$, respectively.
% \begin{displaymath}
% \begin{aligned}
% & {\it r6}.~{\tt cp(Id, Id)} \arrow {\tt cluster(Id, Id)}. \\
% & {\it r7}.~{\tt cp(C, Id)} \arrow {\tt cluster(C, C1)}, {\tt cp(C1, Id)}. \\
% & {\it r8}.~{\tt dp(Id1, Id2, \sumv{D})} \arrow {\tt house(Id1, Col, V1)}, {\tt house(Id2, Col, V2)}, \\
% &\hspace{12em} {\tt D = (V1 - V2) * (V1 - V2)}. \\
% & {\it r9}.~{\tt dc(C1, C2, \minv{Dist})} \arrow {\tt cp(C1, Id1)}, {\tt cp(C2, Id2)}, {\tt dp(Id1, Id2, Dist)}.
% \end{aligned}
% \end{displaymath}
% \end{example} 

==> early_times.tex <==
\section{The early times}

==> language.tex <==
\newtheorem{theorem}{Theorem}
\def\lfp{{\tt lfp}}
\section{Datalog Extensions: Extrema, Count and Sum in Recursive Rules}\label{sec:extrema}

A most significant advance in terms of language and expressive power offereed  by our systems \cite{shkapsky2016big,DBLP:journals/vldb/YangSZ17} is  that they provide a formal semantics and 
efficient implementation  for recursive programs  that use  min, max, count and sum
 in recursion.  We present here an informal summary of  these  advances 
 for which  \cite{ourpaper1} provides a formal in-depth coverage.

% We consider  the situation where recursive  rules define a predicate upon which a constraint
% is applied by the final rule.  

Consider for instance  Example 1,
% and  the final rule $\tt r_3$ specifies that upper-bound constraint ``$\tt  Dy<143$''  must be applied to its
% second argument;  this argument and the variable $\tt Dy$ it contains
% will be refer to as a cost argument  and and a cost variables.
and the goal $\tt is\_min((Y), (Dy))$ in  $\tt r_4$
specifies that we want the min values of $\tt Dy$ for each
unique value of  $\tt Y$ in $\tt path$ defined by rules $\tt r_1$
and $\tt r_2$. Using SQL parlance, we will refer to $\tt Y$  as the group-by variable and to  $\tt Dy$
to the the cost variable, and the same denominations will respectively be applied to the  first and second arguments of $\tt is\_min$.

  \begin{example}[Limited length paths from node a in a directed graph]
  \vspace{-2ex}
 \label{ex:llimited}\inv
 \bldl
\prule{(r_1)~~path(Y, Dy)} {arc(a, Y, Dy), Dy\geq0.}
\prule{(r_2)~~path(Y, Dy)}{path(X,  Dx) , arc(X, Y, Dxy), Dxy\geq0, Dy=Dx+Dxy.}
\prule{(r_3)~~llpath(Y, Cost) } {path(Y, Cost),  Cost<143.~~~~~~~~~~~~~~~~~~}
\prule{(r_4)~~spath(Y, Dy) } {path(Y, Dy),  is\_min((Y), (Dy)).}
\eldl
\end{example}

Thus, $\tt is\_min((Y), (Dy))$ denotes that we want the min values of $\tt Dy$ for each
unique value of  $\tt Y$. %will denote that we seek  the overall min of those $\tt Y$ values.
The special notation used for   $\tt is\_min((Y), (Dy))$ reminds users
and compilers that  this is a special predicate supported by a specialized implementation and the  query 
and optimization techniques  discussed next, and dual observations hold for $\tt is\_max$.
However in terms of  formal  semantics rules with   construct can be viewed as rules using the standard (closed-world)  negation,  whereby the semantics of
 $\tt r_4$ is defined by the following two rules\footnote{This rewriting assumes that there is only 
 one $\tt is\_min$ in our program. In the presence of multiple occurrences, we will need to add a subscript to  
keep them distinct.}.
%Note that the second rule is safe because evaluated in a top-down fashion~\cite{deals}.
\inv
\bldl
\prule{spath(Y, Dy) } {path(Y, Dy),  \neg ismin(Y, Dy).}
\prule{ismin(Y,Dy)}{path(Y, Dy), path(Y, Dy1), Dy1 <Dy.}
\eldl
Expressing our $\tt is\_min$ via negation also reveals
 the  non-monotonic nature of extrema constrains,  whereby this program will treated as a  stratified program, with a "perfect model" semantics, realized by an iterated-fixpoint  computation~\cite{DBLP:conf/iclp/Przymusinski88}. In this computation, 
 $\tt path$ is assigned to a stratum lower than
$\tt spath$ and thus the computation of $\tt path$  must 
complete before the computation of $\tt spath$  via $\tt is\_min$ in $\tt r_4$   can begin.
This stratified computation  can be very inefficient or
even non-terminating when the original graph 
of Example 1 contains cycles.
Thus, much research work was  spent on solving this problem,
before the simple  solution described next emerged and was
used in \bigdatalog to  support graph algorithms with superior performance \cite{shkapsky2016big}.
%their usage in the definition of recursive predicates 
This simple solution  consists in taking the $\tt is\_min$ 
constraint on $\tt path$ in $\tt r_4$ and moving it to the rules 
$\tt r_1$ and $\tt r_2$ defining $\tt path$, producing 
the rules in Example 2.
This rewriting   will be called a {\em transfer} 
%  {\em trasfer } and for  the example a hand it
%  involves  moving the $\tt is\_min$ goal from the final rule $\tt r_4$ to
% the  rules $\tt r_1$ and $\tt r_2$ defining our recursive predicate
of constrain\footnote{In the example at hand we  have conveniently used the  same 
names for  corresponding variables  in all our rules. In general  however, the transfer
 also involves a renaming for  the variable(s)  used in specifying the 
 constraint. For instance,  the $\tt r_3$   constraint  $\tt Cost >143$ is 
 transferred to  $\tt r_1$ and  $\tt r_2$ via 
 the goal  $\tt Dy >143$ added to these two rules.}.

\begin{example}[Shortest path  from node $\tt a$]
\label{ex:shortestpath1}
  \vspace{-2ex}
\bldl
\hspace{-1ex}\prule{(r'_1)~~path(Y, Dy)} {arc(a, Y, Dy), Dy\geq0, is\_min((Y), (Dy)).}
\hspace{-1ex}\prule{(r'_2)~~path(Y, Dy)}{path(X,  Dx) , arc(X, Y, Dxy), Dxy\geq0,Dy=Dx+Dxy,}
\pbody{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}{is\_min((Y), (Dy)) .}
\hspace{-1ex}\prule{(r'_4)~~spath(Y, Dy) } {path(Y, Dy).}
\eldl
\end{example}
While, at the syntactic level, this transfer  of constraint is quite simple, at the semantic level,
 it raises the  following 
two  critical questions: (i) does  the program in Example 2 have
a formal semantics, notwithstanding the fact it uses non-monotonic constructs in recursion,
and (ii)  is it equivalent to the original program, inasmuch as it produces the same  answers for $\tt spath$? 
A positive formal answers  to both  these was provided in \cite{ourpaper1} using the notion of {\em pre-applicability} which is summarized next.
%General conditions for pre-applicability based
%on the Immediate Consequence Operator (ICO) for such rules were discussed in \cite{iclap1} 
%for the rules defining a single recursive predicate. 
 
Let $T$ denote the Immediate Consequence Operator (ICO)
for the rules defining a  recursive predicate\footnote{The 
case of multiple mutually recursive predicates will be
discussed later.}. 
Since our rules are positive, the mapping defined by 
$T$ has a least-fixpoint  $\lfp(T)$  in the lattice of set containment. 
Moreover the property that
$\lfp(T)=T^{\uparrow \omega}(\emptyset)$  allow us to turn this declarative semantics into a concrete one.

%In our previous examples we have only one  recursive predicate, and a constraint $\gamma$ applied to that 
%predicate. But in a more general situation we might have mutually recursive predicates and the constraint 
%$\gamma$ applied to 
Now let $\gamma$ be a constraint, such as a min constraint
or an upper-bound constraint.  Then we have the following important definition:
% Preapplicability is a property is a general property that, in addition to extrema, can be used
%to optimize logic programs in the presence of upper-bound constraints and others as well.

\begin{definition}% {\vspace{-0.4cm} \hspace {1.8cm}\tt :  Preapplicability}
The constraint $\gamma$ is said to be \emph{pre-applicable}
to $T$ when, for every interpretation $I$, we have that: $\gamma(T(I)) = \gamma (T(\gamma (I)))$.
\end{definition}
%$\lfp(T)$ and compute $\gamma(\lfp(T))$. 
For convenience of notation, we will also denote by $T_\gamma$ the
composition of   the function $T$  with the function $\gamma$, i.e.,
 $T_\gamma(I)= \gamma(T(I))$, which will be called the {\em constrained 
 immediate consequence operator} for our program.
 Then, pre-applicability holds whenever $T_\gamma (I)=  T_\gamma( \gamma(I))$.
%
%In particular, we are interested in simple examples, such as  Example1, where  our constraint
%$\gamma$ is applied to a recursive predicate $P$ where $p$ is defined by rules with ICO $T$.
%Then, a sufficient condition for pre-applicability is that pre-applicability holds for each $r$ defining 
%$T$, i.e., it holds for each $T_r$, where $r$ is the ICO defined by rule $r$. 
%In fact we can observe that if $T$ is only defined by non-recursive rules then the pre-applicability 
%property always hold, since  $T_\gamma(\emptyset)= \gamma(T(\emptyset))$.
The following important theorem then follows directly from the definitions~\cite{ourpaper1}:
\begin{theorem}
If the constraint $\gamma$ is pre-applicable to $T$,  and a fixpoint exists such that
$T^{\uparrow n+1}(\emptyset) = T^{\uparrow n}(\emptyset)$ for some integer $n$, then
%converges  after $N$ steps then:
$\gamma(T^{\uparrow \omega}(\emptyset)) = T_\gamma^{\uparrow n}(\emptyset)$.
%If $\gamma$ is pre-applicable to $T$ then  $ \lfp(T_\gamma) =  T^{\uparrow \omega}_\gamma(\emptyset)= \gamma(\lfp(T))$.
\end{theorem}

%Since $T_\gamma$ is also  the ICO of the rules produced by the transfer of 
%the constraint, i.e., rules  $\tt r'_1$ and  $\tt r'_2$ in Example 2,  our theorem
%implies that we can compute these transfer-optimized program as any
%other program, along with semi-naive, magic sets, and other standard Datalog techniques.
%
%Both questions were answered in  \cite{iclp2017submission} where we
% proved that  (i) our  re-written program of Example 2 has indeed a  least-fixpoint semantics, which (ii) produces the same 
% $\tt spath$ answers as the original program in Example 1. 
% %And following \cite{iclp2017submission},
%%use the term {\em pre-applicability} of a constraints to denote the situation where 

 Thus if a constraint is pre-applicable to the given recursive
 rules, its transfer produces  an optimized program 
 having semantics defined by the fixpoint of
its constrained immediate operator of $(T_\gamma)$. In~\cite{ourpaper1} was also shown that the derived fixpoint is also a minimum fixpoint, therefore  possessing
 all the theoretical and computational
properties that follow from such semantics.
For instance, since pre-applicability w.r.t extrema holds  for Example 1,
we conclude  that its optimized version in
Example 2 terminates even if the original graph has cycles.

Now let see why pre-applicability of 
min and max holds for the rules $\tt r_1$
and $\tt r_2$ of Example 1. Pre-applicability holds for $\tt r_1$ since the property always hold for non-recursive rules.
To prove pre-applicability of $\tt is\_min((Y), (Dy))$.
to $\tt r_2$, we can exploit the
properties of its interpreted goals: $\tt Dxy \leq 0, Dy=Dx+Dxy$. 
Indeed, let  $\tt r'_2$  and $\tt r"_2$  be two instances of 
$\tt r_2$  where the
$\tt X$-value in  $\tt r'_2$  is the same as that $\tt r"_2$, but the value of $\tt Dx$ in  $\tt r'_2$,   
is $\leq$ to  that in  $\tt r"_2$. Then
the interpreted goals
compute a $\tt Dy$ value in the head of $\tt r'_2$,   
is $\leq$ to  that of  $\tt r"_2$,
which is thus eliminated by
the outer $\tt is\_min$. Therefore  pre-applications
of $\tt is\_min$ as inner constraint do not  change the actual result.
In \cite{ourpaper1}, 
rules where $\leq$ (resp. $\geq$) cost values in their respective bodies
imply $\leq$ (resp. $\geq$) cost values in their respective heads  are called
deflation-preserving in (resp. inflation-preserving). Then it was
shown that min constraints  are 
pre-applicable to deflation-preserving rules and max 
constraints are pre-applicable to inflation-preserving rules~\cite{ourpaper1}.

% once  $\tt r'_2$ has been found to be true,  the pre-application
% of the  $\tt is\_min$ constraint will cause the failure 
% if  the interpreted goals are  are satisfied in $\tt r' _2$ we
% do not need to consider $\tt r"_2$ since 
% the value of $\tt Dy$  in the head of  $\tt r"_2$  is $\geq$  than those $\tt Dy$ in $\tt r'_2$ and will those be eliminated by 
% $\tt is_min$ constraint at the next step.
% This behavior where smaller  in the rule is called  deflation preserving, whereas the symmetric situation where larger bodies produce large heads was called inflation-preserving.
% Then observe that 
%  during evaluation, because of its larger $\tt Dx$ value  and the $\tt i\_smin$ constraint 
%  $\tt r'_2$ will fail to produce any value  in the head.   But the head values so lost, would
%  have been larger than the head values produced by  $\tt r'_2$  and would thus been eliminated
%  by the $\tt is\_min$ constraint.
%  the min constraint, and  is fine since the final min goal
% would eventually eliminate (i) this larger value in the body, and (ii) that produced by it  in the head
% since it $\leq$ to that produced by $\tt r'_2$.   
%  Thus we have that the  $\tt is\_min$  constraint 
% is pre-applicable  to our deflation preserving rule $\tt r_2$(symmetrically a $\tt is\_max$ constraint
% is pre-applicable to inflation preserving rules.)

Pre-applicability is a general property that applies to different classes of constraints including extrema constraints,  and upper/lower bound
constraints. The latter are also discussed in  \cite{ourpaper1} 
where simple rules  are also given that describe
when these can be  applied in combination. 
The upper-bound
constraint  $\tt Dy <143$ is pre-applicable to rule $\tt r_2$ 
in Example 1  since this  
defines an {\em ascending mapping}. A rule $\tt r$ defines
 ascending mappings when in all
instances of $\tt r$ that satisfy the 
interpreted goals, the value of the cost variable in the head is $\geq$ than all cost variables  in the body. 
% Since upper bound constraints are pre-applicable to rules defining 
% ascending mappings \cite{ourpaper1}  
For instance, constraint $\tt Dy <143$ can be transferred  to rules $\tt r_1$ and $\tt r_2$, producing rules  $\tt r^{\prime}_1$ and $\tt r^{\prime}_2$ of Example 2.
Even after the transfer of this upper bound constraint
$\tt r'_2$ remains deflation-preserving, since lower values of 
the cost argument in the body produce lower values in the head.
Thus if we have the situation where a  final rule 
specifies a conjunct of min and upper-bound constraints on a recursive
predicate the conjunct can be transferred 
to the rules defining the predicate\footnote{The same conclusion is obtained if we
first transfer the min and then  the upper-bound.}.
But, if instead of $\tt Dy <143$ our constraint is a lower-bound, say  $\tt Dy >16$,
then this cannot be pre-applied to 
the rules in Example 2, since these do not define an ascending mapping.  Symmetrically,
we can  transfer   $\tt Dy >16$ to the rules in Example 1, which also define an ascending mapping, but then
the resulting rules are no-longer deflation preserving 
and we cannot transfer the min.
Thus, if we have both  a  $\tt is\_min$ and a lower-bound constraint, we can transfer one or the other 
but not both.  Symmetric properties hold for the max.

The optimization here described apply to a very large set of programs of practical interest, and are a crucial factor in the superior performance of \bigdatalog.
Indeed,  we have  here a  significant generalization of the fixpoint semantics of logic programs
where users can now write powerful algorithms by  using extrema in recursive rules. Our experience 
show that these programs can be more appealing to the intuition than the equivalents
stratified programs where extrema are used as postconditions. Naturally, the compiler verifies
the semantic correctness of these programs by removing them from the rules and asking whether they
are pre-applicable to the rules they were removed from.  If so, the original
program is executed, otherwise an error message is generated.
%!TEX root = pods17.tex
\inv\subsection{Monotonic Count}
\label{sec:count}
%\section{From Count to Monotonic Count and Back}
% \label{sec:aggregates}
% The need to use aggregates in Datalog applications  has motivated much research work seeking to support extrema and count aggregates in Datalog.
% It is important therefore that we understand the relationship between the  different approaches
% and how they dovetail at the theoretical level and practical level.  The next example recasts in
% our syntax the one proposed by
%  Ross and Sagiv \cite{ross1992monotonic} to illustrate the problems caused by traditional aggregates in recursion:
% \begin{example}[A program with multiple minimal models]
% \label{ex:ross_sagiv_example}
% \inv\bldl
% \pfact{p(b).~q(b).} {}
% \prule{cq(count \langle X \rangle)} {q(X).~~~~~~~}
% \prule{cp(count \langle Y \rangle)}  {p(Y).}
% \prule{p(a)}{\hspace{-1.4cm} cq(CC), CC=1. ~~~~~~~~~~~~~~~~~~}
% \prule{q(a)}{\hspace{-1.4cm} cp(CC), CC=1.~~~~~~~~~~~~~~~}
% \eldl
% \end{example}

% For this program we have two least fixpoints, which are also minimal models.
% The  first  consists of (i):   $\tt p(b),  cp(1),$ $\tt   q(a), q(b), cq(2)$ and
% the second consists of (ii):  $\tt  p(a), p(b),$ $\tt cp(2),$ $\tt   q(b),   cq(1)$.
% While logic programs with multiple canonical models can be handled
% in the framework of stable models and answer-set \cite{Gelfond88thestable},
% Datalog researchers have always sought approaches that preserve the
% traditional semantics  and desirable computation properties
% of Horn clauses~\cite{ullman1990principles}.
% In particular the approach
% proposed in \cite{mazuran2012extending} have been incorporated
% in many systems \cite{shkapsky2015optimizing,yang2015parallel,shkapsky2016big,yang2016scaling} including the BigDatalog system for
% Apache Spark \cite{shkapsky2016big}, where
% they  have enabled the expression and support of graph algorithms more
% efficient than those written in GraphX. Thus, we  investigate next how this
% approach interacts with the optimization  techniques based on pre-applying
% extrema constraints previously discussed.


At the core of the approach proposed in \cite{mazuran2012extending}
there is the observation that the cumulative version of standard count is 
monotonic in the lattice of set containment. Thus they introduce 
 $\tt mcount$  as the 
aggregate function that returns all natural numbers up to the cardinality of the set.
%  Therefore, the standard
% least-fixpoint semantics holds for programs that use the continuous count $\tt mcount$ in recursive rules. 
The use of $\tt mcount$ in actual applications
is illustrated by the following example that is similar to one
proposed in \cite{ross1992monotonic}.

%In fact, if  in Example \ref{ex:ross_sagiv_example} we replace the $\tt count$ with $\tt mcount$, we obtain
%a unique least fixpoint and minimal model: $\tt p(a), p(b), cp(1)$, $\tt cp(2), q(a), q(b), cq(1), cq(2)$.  Naturally, enumerating all
% integers till the max can be inefficient, but this can be solved by  adding a max constraint in the
% extraction rule, as illustrated by the following example taken from \cite{ross1992monotonic}.

\begin{example}[Join the party once you see that three of your friends have joined]
\label{ex:attend1}
The organizer of the party will attend, while other people
will attend if the number of their friends attending 
is  greater or equal to 3, i.e., ${\tt Nfx \geq 3}$.
%\bldl
%\prule{fcount(Y,  max \langle CC \rangle )}{fcount(Y,  CC).}
%\prule{ cntfriends(Y,  mcount \langle X \rangle)} {\tt attend(X), friend(X, Y).}
%\eldl
\bldl
\prule{ attend(X)}{~~~~organizer(X).}
\prule{attend(X)}{~~~~~cntfriends(X, Nfx), Nfx \geq 3.}
%\prule{cntfriends(Y, \mcntv{X})}{\hspace{-0.2cm}attend(X), friend(X, Y)}
\prule{cntfriends(Y, N)}{attend(X), friend(Y,X), mcount((Y),(X), N ).}
\eldl
\inv\inv
\end{example}

Here too we use the body notation for our monotonic 
count-distinct  aggregate, $\tt mcount$, where   
its first argument  $\tt (Y)$  is  the group-by argument; its second $\tt (X)$, is the 
\emph{count  argument}, and the third is
the result of the count aggregate. The count argument contains one or more variables,
whereas the  group-by argument can contain zero or more variables.

As described in \cite{mazuran2012extending}, the semantics of  $\tt mcount((Y), (X), N)$
can be reduced to that of Horn Clauses.
%\footnote{
%\inv\inv
%\bldl
%\prule {mcount(Y,  N)}{cntall(Y, \_, N).}
%\prule {cntall(Y,   X, 1)}{attend(X), friend(X, Y).}
%\prule{cntall(Y, [X|T], N1 )}{attend(X), friend(X, Y), cntall(Y, T, N), notin(X, T), N1=N+1.}
%\eldl
%where $\tt notin$ is defined without using negation, as follows:
%\inv
%\bldl
%\pfact{notin(Z, [~]).}{}
%\prule{notin(Z, [V|T])}{Z \neq V , notin(Z, T).}
%\eldl
%This formulation is obviously inefficient since the progressive count 
%is computed on every possible permutation of the given set although 
%the same result is returned for each permutation.} % a property used
%%by the built in aggregate that will only use the most easily materialized
%%permutation.} 
%The use of mcount in recursion
%allows us to express programs, such as counting
%paths between two nodes, that are not expressible using the standard aggregates
%in stratified programs \cite{mumick1995expressive}.
Now,  $\tt mcount$ is a monotonic aggregate function and as such is fully compatible with standard  semantics of Datalog 
and its optimization techniques, including the transfer of extrema, discussed in the previous section.

%
%  and  it also has unique properties that play a major role in
%its interaction with comparison and extrema constraints and their combined
%use in practical applications.
% In particular,
%a first observation to be made is that,  upper-bound constraints
%comparing the results of mcount with positive integers are quite useful.
%However, lower-bound constraints upon  mcount serve no useful purpose, since they
%are always true when the bound is a positive integer,  and always false when
%the bound is a non-positive integer.

%Next we address the question of whether we
%can pre-apply extrema constraints to rules using mcount.
%The rules in our example are inflation-preserving and thus we can
%replace mcount with count, which produces a slightly more efficient computation.
%By  the query goal  $\tt attend(N)$ the
%program in Example \ref{ex:attend1} will return the names of the people 
%who will attend the party. To find out the 
%number of friends each attendee will have at the party,
%we can use the query goal  $\tt  cntfriends(Y, X)$, which however
%is likely to return many  answers, since
%for an attendee  with $k$ friends it will return
%his/her name $k$ times.  
We can now use the following rule, to
 find  the people who come to the party and  the number of friends they will see there:
\footnote{This will show the  persons who have friends at the party and their total
number. To eliminate people who only have one or two friends and thus will not
attend, we will have to include the additional final condition: $\tt N \geq 3$.}

\cldl
\prule{fcount(Y, N)} {cntfriends(Y, N), is\_max((Y), (N)).}
\eldl

Here we have two mutually recursive predicates, but si
since $\tt is\_max$  in the final rule has applied to 
$\tt cntfriends(Y, N)$ we only transfer it to 
the  rule that has 
$\tt cntfriends$ as its head, where $\tt is\_max$ and 
$\tt mcount$ are combined into
the standard  $\tt count$, yielding the following program.

\begin{example}[Join the party once three of your friends have joined using standard count]
\label{ex:attend5}\inv
\cldl
\prule{ attend(X)}{organizer(X).}
\prule{attend(X)}{cntfriends(X, Nfx), Nfx \geq 3.}
%\prule{cntfriends(Y, \mcntv{X})}{\hspace{-0.2cm}attend(X), friend(X, Y)}
\prule{cntfriends(Y, N)}{attend(X), friend(Y,X),count((Y),(X), N ).}
\prule{fcount(Y, N)} {cntfriends(Y, N).}
\eldl
\inv\inv
\end{example}

The program so obtained is more efficient than the regular program. 
Moreover, we found that
in many algorithms, the regular count is more appealing to users than monotonic count; therefore they should be allow to use count in recursion as long as the program has a least  fixpoint semantics~\footnote{
Here too, when presented with this program, the  compiler  
transfers back the  max condition to the rule calling $\tt cntfriends$, to see
if it is pre-applicable to the rule where count has been replaced by mcount. If this check succeeds then the original program is executed, otherwise an error message is  generated.}.

So far, we have used the tail notation for aggregates, but \bigdatalog in fact uses the head notation, which
appears to be easier for users because it achieves uniformity 
of notation across different aggregates. The transformation from tail-notation back to head
notation is straightforward. For our example the third rule can be re-written as follows:
\bldl
\prule{cntfriends(Y, count\langle Y \rangle)}{attend(X), friend(Y,X).}
\eldl
\inv
\subsection{From Monotonic SUM to Regular SUM } 
The notion of monotonic sum, i.e.,  $\tt msum$, for positive numbers
was  introduced in \cite{mazuran2012extending}  
using the fact that the semantics  $\tt msum$ and $\tt sum$ for positive 
numbers can be easily reduced to that of $\tt mcount$ and $\tt count$, respectively,
as  illustrated by the following example computing the total number of  each part  that is 
available in each city
by adding up the quantities held in each store  of that city.

\cldl
\prule {\hspace{-3ex}pCnt\_InCity(Pno, City, sum\langle Qty, Store \rangle)}   {pqs(Pno, Store, Qty),  cs(Store, City).}
\eldl

Here, the sum  is computed by adding up the
$\tt Qty$ values,  but  the presence of $\tt Store$ makes sure 
that  all the repeated occurrences of the same $\tt Qty$ are considered in the addition,
rather than being ignored as a set semantics would imply.
The results returned by this rule are the same as those returned by the following  rule
where $\tt posint$ simply enumerates the positive integers up to  $\tt Qty$:

\bldl
\prule {partCnt\_InCity(Pno, City, count \langle Eq, Store\rangle)}   {}
\pbody{\hspace{3cm}} {pqs(Pno, Store, Qty),  cs(Store, City),posint(Qty, Eq).}
%\prule{partCnt\_InCity(Pno, City, max<Qty>0}{enumerateAll(Pno, City, CQy.}
\eldl

Then consider the following example where we want to count the distinct paths
connecting any pair of node in the graph:

\cldl
\prule{cpath(X, X, 1)} {arc(X, \_).}
\prule{cpath(X, Z, sum \langle Cxy, Y \rangle} { cpath(X, Y, Cxy), arc(Y, Z).}
\eldl

%The operational semantics of this program is simple. For instance, 
%If  we have arcs between the following pairs of nodes: (a,b), (b, c), (a,c), (c, d)
%the fixpoint iteration will return:
%(a,a, 1), (b,b,1), (c, c, 1)
%(a,b, 1), (b, c, 1), (a, c, 1)
%(a, c, 2) (b, c, 1)

Then the semantics of our program is defined by its equivalent rewriting 
\bldl
\prule{cpath(X, Y, 1)} {edge(X, Y).}
\prule{cpath(X, Z,  count \langle Y, Ixy \rangle)}  {cpath(X, Y, Cxy), edge(Y, Z), posint(Cxy, Ixy).}
 \eldl                           

Thus the compiler will first check if this program has a  least fixpoint by viewing  count
as an mcount to which a max has been transferred from a final rule and asking if the
pre-applicability condition holds. The answer is here positive, and thus 
.the compiler will execute the much more efficient original program.
While we have here used integers for cost arguments, floating point 
numbers can be handled in the same fashion \cite{mazuran2012extending}.
%\clearpage
 





==> middle_ages.tex <==
\section{The Middle Ages}

2006-ish? declarative networking?

==> moreapp.tex <==
\subsection{New applications and future developments}

==> renaissance.tex <==
\section{The Renaissance and its many splendors}



\section{Monotonic Aggregation}

\input{multicore}
\input{bigdatalog}
\input{applications}
\input{moreapp}
